Fast Parametric Model Checking through Model Fragmentation

Parametric model checking (PMC) computes algebraic formulae that express key non-functional properties of a system (reliability, performance, etc.) as rational functions of the system and environment parameters. In software engineering, PMC formulae can be used during design, e.g., to analyse the sensitivity of different system architectures to parametric variability, or to find optimal system configurations. They can also be used at runtime, e.g., to check if non-functional requirements are still satisfied after environmental changes, or to select new configurations after such changes. However, current PMC techniques do not scale well to systems with complex behaviour and more than a few parameters. Our paper introduces a fast PMC (fPMC) approach that overcomes this limitation, extending the applicability of PMC to a broader class of systems than previously possible. To this end, fPMC partitions the Markov models that PMC operates with into \emph{fragments} whose reachability properties are analysed independently, and obtains PMC reachability formulae by combining the results of these fragment analyses. To demonstrate the effectiveness of fPMC, we show how our fPMC tool can analyse three systems (taken from the research literature, and belonging to different application domains) with which current PMC techniques and tools struggle.

==> Algorithms/Fragment_Grow.tex <==


\begin{algorithm}[th!]
    \label{algorithm:fragmentgrow}
    \footnotesize
    \SetKwInOut{Data}{Data}
    \SetKwInOut{Result}{Result}
    \Data{Graph $G(V,E)$, An input vertex $w$ and Stack $S$}
    \Result{A set of vertices stored in $S$}
    \vspace{0.3cm}
    \tcc{Growing from incoming transitions only applies to vertices that is not the starting state of a fragment}
    \If{$w$.start != true}{
        \For{each (i,w) in E}{
            \eIf{All $i$.fragment == NULL}{
                S.add($i$)
            }{
            \tcc{Set a fragment using a single vertex - $w$}
            $w$.fragment = unique index
            
            $w$.start = true
            
            $w$.end = true 
            }
        
        }
    }
    \vspace{0.3cm}
    \tcc{Growing from outgoing transitions applies to all vertices}
    \For{each (w,o) in E)}{
        \eIf{$o$.fragment == NULL}{
            S.add($o$)
        }{
            \tcc{The method and validity of creating an auxiliary vertex is discussed in ...}
            Create an auxiliary vertex $o'$ between $o$ and $v$
            
            S.add($o'$)
        }
    }
    \caption{fragmentgrow()}
\end{algorithm}

==> Algorithms/Fragmentation.tex <==
%!TEX root = conference_main.tex

\begin{algorithm}[h!]
\label{algorithm:fragmentation}

    \footnotesize
    \SetKwInOut{Data}{Data}
    \SetKwInOut{Result}{Result}
    \Data{Graph $G(V,E)$, State, $P$, for which property will be checked}
    \Result{A set of vertices that have been fragmented}
    
    Const int MAX
    
    index := 0
    
    $S$ := an empty stack
    
    V.fragment = NULL
    
    P.fragment = index
    
    index++
   
    \For{each $v$ in $V$}{
        \If{ $v$.fragment == NULL}{
            $v$.start = true
            
            $v$.fragment = index
            
            \tcc{This funcition is discribled in Algorthim 2}
            fragmentgrow($v$)
        }
        \vspace{0.2cm}
        \While{$S$ is not empty}{
            
            s = S.pop
          
            \eIf{$CurrentFragment.size < MAX$}{
               \eIf{s in S is not a valid ending point of a fragment}{
                    fragmentgrow($s$)
                } {
                    $s$.end = true
                }
            }{
    
                \eIf{s in S is not a valid ending point of a fragment}{
                \tcc{The modification is dicussed in Section...}
                    \eIf{s can be modified to be an ending point}{
                        
                        perfrom the modificiation
                        
                        $s$.end = true
                    }{
                        fragmentgrow($s$)
                    }

                } {
                    $s$.end = true
                }
            
            
            
            }
            $s$.fragment = index
        }
        \vspace{0.2cm}
        \tcc{Check if the formed fragment is valid}
        \eIf{the formed fragment satisfies all the policies}{
            A fragmentation is formed
        }{
        \tcc{Restore all the vertices in the current fragment}
            \For{each $w$ that w.fragment == index}{
                
                $w$.fragment = NULL
            }
            \tcc{Set the fragment with a single vertex}
            $v$.fragment = index
            
            $v$.start = true
            
            $v$.end = true
        }
        
        index++
    }
    \caption{Fragmentation}
\end{algorithm}

==> Tables/Approach_State_policy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\footnotesize
\centering
\caption{Policies for each types of states of being a valid fragment}
\label{Table:Approach_Policy}
\begin{tabular}{|c|cc|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Fragment and State\\ Category\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}{[}Min, Max{]} number of such \\ states can be in the fragment\end{tabular}} &
  \textbf{Policy for incoming transitions} &
  \textbf{Policy for outgoing transitions} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}} \\ Fragment with \\ multiple states\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Input\\ state\end{tabular}}} &
  {[}1,1{]} &
  No rules &
  To the states with the same fragment \\ \cline{2-5} 
 &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Inner\\ state\end{tabular}}} &
  {[}0,n/a{]} &
  From the states with the same fragment &
  To the states with the same fragment \\ \cline{2-5} 
 &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Output\\ state\end{tabular}}} &
  {[}1,n/a{]} &
  \multicolumn{1}{l|}{From the states with the same fragment} &
  \begin{tabular}[c]{@{}c@{}}To the states with the \textbf{different} fragment \\ or\\ To the input state of the same fragment\end{tabular} \\ \hline
\multicolumn{2}{|c|}{\textbf{Fragment with single state}} &
  {[}1,1{]} &
  No rules &
  No rules \\ \hline

\end{tabular}
\end{table*}

==> Tables/Hyperparameter_sensitivity_table.tex <==
\begin{table*}[]
\begin{tabular}{c|c|c|c}
\hline
\textbf{Max Value Used} & \textbf{Time (s)} & \textbf{\#operation} & \textbf{\begin{tabular}[c]{@{}c@{}}\# states in\\ abstract model\end{tabular}} \\ \hline
2  & 8.777   & 6468   & 18 \\
3  & 7.532   & 6468   & 18 \\
4  & 4.605   & 1456   & 13 \\
5  & 4.469   & 1456   & 13 \\
6  & 4.436   & 1456   & 13 \\
7  & 4.551   & 3279   & 9  \\
8  & 4.748   & 3279   & 9  \\
9  & 4.772   & 3279   & 9  \\
10 & 4.694   & 3279   & 9  \\
11 & 4.906   & 3279   & 9  \\
12 & 4.425   & 3279   & 9  \\
13 & 4.617   & 3279   & 9  \\
14 & 4.463   & 3279   & 9  \\
15 & 4.555   & 3279   & 9  \\
16 & 8.214   & 8536   & 8  \\
17 & 8.116   & 8536   & 8  \\
18 & 7.924   & 8536   & 8  \\
19 & 8.004   & 8536   & 8  \\
20 & 8.011   & 8536   & 8  \\
21 & 14.970  & 15845  & 7  \\
22 & 98.404  & 78952  & 4  \\
23 & 97.898  & 78952  & 4  \\
24 & 96.826  & 78952  & 4  \\
25 & 97.108  & 78952  & 4  \\
26 & 120.800 & 78952  & 4  \\
27 & 102.624 & 78952  & 4  \\
28 & 177.317 & 124854 & 3  \\
29 & 176.290 & 124854 & 3  \\
30 & 180.984 & 124854 & 3  \\ \hline
\end{tabular}
\end{table*}
